Seeing to Generalize: How Visual Data Corrects Binding Shortcuts

Vision Language Models (VLMs) are designed to extend Large Language Models (LLMs) with visual capabilities, yet in this work we observe a surprising phenomenon: VLMs can outperform their underlying LLMs on purely text-only tasks, particularly in long-context information retrieval. To investigate this effect, we build a controlled synthetic retrieval task and find that a transformer trained only on text achieves perfect in-distribution accuracy but fails to generalize out of distribution, while subsequent training on an image-tokenized version of the same task nearly doubles text-only OOD performance. Mechanistic interpretability reveals that visual training changes the model's internal binding strategy: text-only training encourages positional shortcuts, whereas image-based training disrupts them through spatial translation invariance, forcing the model to adopt a more robust symbolic binding mechanism that persists even after text-only examples are reintroduced. We further characterize how binding strategies vary across training regimes, visual encoders, and initializations, and show that analogous shifts occur during pretrained LLM-to-VLM transitions. Our findings suggest that cross-modal training can enhance reasoning and generalization even for tasks grounded in a single modality.

==> sections/01_intro_old.tex <==
\section{Introduction}

% The ability to reliably associate attributes with entities, known as \textit{binding}, is fundamental to in-context reasoning. Yet, despite their scale, Large Language Models (LLMs) often rely on fragile heuristics to perform this task. Unlike humans, who bind properties to objects via semantic identity, Transformers often default to processing sequences as fixed positional grids, struggling to distinguish "who is who" without explicit structural guidance \cite{gur-ariehMixingMechanismsHow2025a}. This reliance on position limits their ability to generalize to complex, noisy, or unstructured settings where the rigid linear order of text breaks down. In this work, we investigate the mechanistic origins of this fragility and demonstrate how multimodal training can fundamentally rewire the model to overcome it.

% Recent mechanistic interpretability research has identified that LLMs employ a \textit{mixture of mechanisms} for binding \cite{gur-ariehMixingMechanismsHow2025a}. In simple or structured contexts, models default to a \textbf{Positional Mechanism}, essentially "counting" indices to link the $n$-th attribute to the $n$-th entity. This mechanism is inherently brittle: it fails when the sequence order is disturbed or when bidirectional retrieval is required. Only when this signal degrades do models supplement it with a more robust \textbf{Lexical Mechanism} (retrieving by semantic identity) or \textbf{Reflexive Mechanism}.

% We hypothesize that the structural constraints imposed by visual data force models to abandon these brittle heuristics in favor of robust, identity-based mechanisms. Research on "Grounding IDs" suggests that external visual cues induce latent identifiers that bind objects to specific regions, bridging the gap between visual perception and textual description \cite{hasaniUncoveringGroundingIDs2025}. Furthermore, predictive architectures like JEPA have been shown to mitigate binding failures by forcing theperkjkjkjkjk model to predict in a semantic space, treating objects as distinct entities rather than surface-level tokens \cite{wangReversalCurseBinding2025,chenVLJEPAJointEmbedding2025}. We propose that visual training acts as a similar forcing function: because images lack the strict linear order of text, they compel the model to abandon simple index counting and develop internal states functionally analogous to Grounding IDs.

% To test this hypothesis, we adapt the interchange intervention method proposed in \textit{Mixing Mechanisms} \cite{gur-ariehMixingMechanismsHow2025a} to our single-hop binding task (Figure 1). We refine the definition of the positional mechanism by distinguishing between two modes: \textbf{Positional Context} (relying on the object's position in the source) and \textbf{Positional Binding} (relying on position in the query). This distinction reveals that the text-only models in our study heavily over-rely on \textbf{Positional Context}, explaining their failure to generalize to reordered or reversed sequences.

% In this work, we show that this reliance is an artifact of data modality, not architecture. We find that models trained on pure text converge to a brittle \textbf{Positional Context} solution that collapses under reordering or noise (Figure 2). Even when we explicitly train models on text with noise and distractors to discourage this behavior, they only partially adapt; while they develop a wider mixture of mechanisms, they remain predominantly reliant on \textbf{Positional Context}. However, by introducing visual grounding tasks, we drive a complete phase transition in the model's internal circuitry. Multimodal training acts as a structural regularizer, suppressing the "lazy" positional mechanism and forcing the emergence of a robust \textbf{Lexical Mechanism}. The model learns to merge attribute information directly into the token identity, creating stable internal representations that generalize robustly out-of-distribution, handling noise, unseen numbers of items, and modifications in the order of attributes.

% We validate this "mechanism shift" in state-of-the-art open-weights models. Comparing Qwen 2 (text-only) with Qwen 2-VL (vision-language), we observe distinct mechanistic signatures (Figure 3). Using our modified interchange experiment and linear probes, we show that the vision-language model merges color and context information more effectively and earlier in the network. This suggests that visual pre-training fundamentally rewires the text processing algorithm, moving the model from a fragile reliance on positions to a robust understanding of identities.

% Large language models (LLMs) are known for their capacity to perform in-context reasoning \cite{brownLanguageModelsAre2020d}. Increasingly this has been associated with the ability for a model to dynamically associate attributes with entities, an ability known as \textit{binding}. This is a fundamental skill that arises from psychology \cite{treismanBindingProblem1996}....

% While LLMs appear to have the requisite skill to solve binding problems, it has been found that they rely on different mechanisms depending on the length of the prompt, number of distractors, number of entities, etc \cite{gur-ariehMixingMechanismsHow2025a, fengHowLanguageModels2024a}.

% The capacity to dynamically associate attributes with entities, known as \textit{variable binding}, is a fundamental prerequisite for compositional thought. Originating in cognitive psychology as the ``Binding Problem'' \cite{treismanBindingProblem1996}, this capability has historically served as the dividing line between classical symbolic architectures and neural networks. Classical systems implement binding trivially via explicit pointers and addressable memory, enabling systematic generalization \cite{wuHowTransformersLearn2025}. In contrast, connectionist models have long been scrutinized for their potential inability to replicate this systematicity without explicit symbolic machinery, a tension that remains central to the field \cite{wuHowTransformersLearn2025}.

% With the rise of Large Language Models (LLMs), this debate has evolved. LLMs demonstrate a remarkable ability to perform in-context reasoning \cite{brownLanguageModelsAre2020d}, appearing to perform variable binding ``on the fly.'' However, it remains an open question whether these models have genuinely acquired robust symbolic machinery or are merely approximating reasoning through statistical shortcuts \cite{tangLargeLanguageModels2023}. Recent mechanistic analyses suggest that LLMs have not settled on a single mechanism to solve these tasks. It has been shown that LLMs use a mixture of mechanisms, denominated ``positional,'' ``lexical,'' and ``reflexive,'' with models shifting between these three mechanisms depending on factors such as the number of distractors and context length \cite{gur-ariehMixingMechanismsHow2025a, fengHowLanguageModels2024a}.

% In this work, we argue that in the linear regime of structurally consistent pure text training, models frequently converge to a less robust mechanism we denote as ``context positional.'' This mechanism identifies entities by their absolute sequence rank in the context section of the prompt, rather than their semantic identity. In the theoretical framework of Distributional Projection, this corresponds to a dominance of ``Position-Position'' ($PSP^T$) projections over ``Content-Content'' ($QSQ^T$) projections \cite{mehtaSelfAttentionDistributionalProjection2025}. This reliance on positional heuristics corresponds to the intermediate developmental stages observed in symbolic learning, where models employ shallow, line-based shortcuts rather than developing the ``addressable memory'' required for systematic processing \cite{wuHowTransformersLearn2025}. While effective for in-distribution text, this behavior is inherently brittle; when the positional grid is perturbed by noise or sequence scaling, the reasoning chain collapses \cite{gur-ariehMixingMechanismsHow2025a}.

% We investigate whether the introduction of the visual modality can fundamentally alter this mechanistic pathology. Unlike text, which is strictly sequential, visual scenes are structurally permutation invariant; a visual patch at coordinates $(0, 0)$ is not causally ``prior'' to a patch at $(10, 10)$. We hypothesize that this invariance acts as a structural regularizer for the attention mechanism. To test this, we employ a curriculum of ``Equivalent Prompts,'' where textual attributes are substituted with visual counterparts in syntactically identical structures. This approach allows us to isolate the effect of the modality constraint on the underlying binding circuit, assessing whether the permutation invariance of the visual input forces the model to abandon rank-based pointers in favor of robust, content-addressable binding mechanisms.

% To rigorously characterize the resulting mechanistic shift, we introduce a suite of targeted interpretability experiments. First, we adapt the interchange intervention technique to the multimodal setting, allowing us to causally map the flow of attribute information and distinguish between heuristic and systematic binding strategies. Second, we employ attention knockout experiments to identify the specific token connections responsible for variable binding and to determine if the mechanism is distributed or localized. Third, we utilize linear probes trained on the residual stream to detect the emergence of ``Lexical Accumulation,'' investigating whether the model physically stores attribute information within entity tokens. Finally, we perform a cosine similarity analysis between the hidden states of our Text-Only and Vision-Tuned models when processing identical text inputs. This allows us to quantify the geometric divergence of the representations and verify whether the visual training induces a topological rotation of the text manifold away from the positional subspace.

% Our investigation aims to challenge the prevailing ``Inheritance Hypothesis'' in Vision-Language Model (VLM) research, which posits that VLMs largely preserve the task representations of their text-only backbones \cite{luoVisionLanguageModelsCreate2025}. By analyzing whether our model aligns vision to the existing text mechanism or fundamentally restructures the text representation itself, we provide new insights into the role of cross-modal training in inducing robustness. Furthermore, we explore the potential of this mechanistic restructuring to resolve fundamental reasoning failures such as the ``Reversal Curse'' \cite{berglundReversalCurseLLMs2024}, connecting our findings to recent work on Joint-Embedding Predictive Architectures (JEPA) \cite{wangReversalCurseBinding2025, chenVLJEPAJointEmbedding2025} and the emergence of symmetric grounding identifiers \cite{hasaniUncoveringGroundingIDs2025}.

% - A central goal in machine learning is to build models that generalize. 
% - In the recent past, models have been tremendously successful by using increasingly large amounts of data in training. 
% - This is in line with the central assumptions of machine learning algorithms that assume that training and test data distribution are iid; thus, there is a need for a larger amount of training data to cover the complete space of possible data points.
% - In real-life settings, this assumption is flawed; various conditions, including limited computational resources, sampling biases, and others, make it impossible to access the complete data distribution. Thus, there is a need for models that are robust to unknown parts of the distribution or that generalize OOD.
Out-of-distribution (OOD) generalization remains a central and longstanding challenge in machine learning, as it probes a model’s ability to maintain reliable performance beyond the conditions observed during training.
Despite remarkable progress in in-distribution (ID) benchmarks, modern neural networks frequently exhibit brittle behavior when exposed to distributional shifts or novel setting \cite{pmlr-v139-koh21a,wang2022generalizing,yang2023out}.
A well-studied manifestation of this limitation is their difficulty in generalizing to longer or more complex inputs than those encountered during training \cite{lake2017original-scan,bastings2018NACS, ruis2020gscan,zhang2022unveiling,saparov2023testing,zhou2024what}, even when the underlying task structure remains unchanged.

A key reason for this fragility is that, in the absence of strong inductive biases, learning systems tend to rely on domain-specific shortcuts or spurious correlations that are predictive in the training distribution but unstable across environments \cite{zhu2016object,geirhos2020shortcut,taori2020measuring,xiao2021noise,ming2022impact}.

Multi-modal training is frequently proposed as a mechanism to mitigate this issue, learn transferable features \cite{alayrac2020self,morgado2021audio}, and promote robustness \cite{radford2021clip}.
By forcing a model to operate across different modalities, it is hypothesized that it discourages reliance on spurious, modality-specific features that may be over-represented in the training data, encourages a more accurate estimation of the underlying latent space representations, and consequently improves out-of-distribution generalization \cite{huang2021makes,xue2024understanding}.

\commentrt{íba recontento leyendo la intro hasta que llegué a este párrafo. Sale de la nada. Es un cambio muy grande de tema. Entiendo que es una transición difícil porque tenemos que meter la idea de binding. Pero hay que mejorar esta transición :)}
A critical capability underlying such reasoning is \textit{variable binding}—the capacity to dynamically associate attributes with entities (e.g., binding `color` to `shape`) and retrieve them for downstream computation (Fodor \& Pylyshyn, 1988; Smolensky, 1990). While fundamental for compositional thought, the specific neural mechanisms LMs employ to solve binding tasks remain debated. Recent work indicates that models utilize a complex mixture of strategies, ranging from positional heuristics to lexical lookups (Feng et al., 2024; Prakash et al., 2024; Gur-Arieh et al., 2025). However, understanding precisely how these mechanisms operate is difficult; LMs often exhibit remarkable resilience to interventions, dynamically shifting between redundant mechanisms to maintain performance (Gur-Arieh et al., 2025). Consequently, it remains unclear which of these internal strategies promotes robust generalization and how training data shapes their emergence.

By forcing a model to operate across heterogeneous modalities, it is hypothesized that the shared supervision constrains the solution space, discouraging reliance on spurious correlations or modality-specific heuristics that may be over-represented in the training data, and instead promotes the discovery of more stable latent representations that capture the underlying generative factors of the task. This cross-modal alignment acts as a regularizer on the representation space, leading to more accurate and semantically grounded embeddings, which in turn improves robustness and out-of-distribution generalization

In this work, we show evidence that training across multiple modalities can actively foster more robust internal mechanisms in neural networks. Concretely, we consider a setting in which a model initially trained on a language-based version of a task is subsequently trained on an image-based instantiation of the same underlying problem and then brought back to the language modality. We show that this cross-modal training trajectory leads to consistent improvements in out-of-distribution performance, most notably in the ability to generalize to longer inputs than those observed during training. This finding indicates that exposure to a different modality does not merely transfer superficial representations but can reshape the computational strategies the model relies on, resulting in stronger forms of generalization. Importantly, we observe that this effect is not restricted to a single architecture or configuration but is prevalent across state-of-the-art models.

Beyond performance gains, we further investigate the underlying causes of this improvement by analyzing the internal mechanisms learned by the models. In particular, we study how models bind entities from the context to construct their predictions, using a combination of probing techniques, controlled interventions, and attention knock-out. Our results reveal that image-based training induces a qualitative shift in the binding strategy employed by the model, moving from a predominantly positional mechanism, which relies on surface-level ordering and local cues, to a more symbolic or lexical mechanism that operates over abstract entity representations. This transition is critical, as symbolic binding is substantially more stable under input transformations such as length extrapolation. By characterizing these mechanisms in detail, we provide new insight into the computations underlying different forms of generalization and offer a concrete explanation of how multi-modal training can reshape a model’s internal structure in ways that directly support improved OOD robustness.

